Nonconvex Optimization Meets Low-Rank Matrix Factorization: An Overview

Substantial progress has been made recently on developing provably accurate and efficient algorithms for low-rank matrix factorization via nonconvex optimization. While conventional wisdom often takes a dim view of nonconvex optimization algorithms due to their susceptibility to spurious local minima, simple iterative methods such as gradient descent have been remarkably successful in practice. The theoretical footings, however, had been largely lacking until recently. In this tutorial-style overview, we highlight the important role of statistical models in enabling efficient nonconvex optimization with performance guarantees. We review two contrasting approaches: (1) two-stage algorithms, which consist of a tailored initialization step followed by successive refinement; and (2) global landscape analysis and initialization-free algorithms. Several canonical matrix factorization problems are discussed, including but not limited to matrix sensing, phase retrieval, matrix completion, blind deconvolution, robust principal component analysis, phase synchronization, and joint alignment. Special care is taken to illustrate the key technical insights underlying their analyses. This article serves as a testament that the integrated consideration of optimization and statistics leads to fruitful research findings.

==> extensions.tex <==
\section{Extensions}

Other related nonconvex optimization problems, including dictionary learning, tensor models, neural networks,
learning mixture models \cite{yi2014alternating} and robust subspace clustering




==> literature.tex <==


%\subsection{Literature}


%nonconvex matrix completion: \cite{sun2016guaranteed}

 


% saddle points in neural networks \cite{dauphin2014identifying}
 
\subsection{State-of-the-art} 

Broadly speaking, there're two lines of active research in studying the behavior of nonconvex optimization for statistical estimation. The trend highlights synergy between statistics and optimization, where on one end, we want the solution of a specific optimization procedure to possess desirable statistical properties, and on the other end, we want the algorithmic choice of computation be informed by statistical models.

{\em Landscape and initialization-free analysis:} The first is an algorithm-independent approach, where the goal is to characterize the ``landscape'' of the loss functions over the entire parameter space used in specific problems, such as the types of critical points and the curvatures of the loss surface. These landscape properties are useful in determining the difficulty of global optimization. Powered by proper signal models, it turns out that we can identify a large family of problems with benign landscape, that is in a nutshell, problems without ``bad'' local minima; and moreover, all saddle points that are not local minima have descent directions that strictly decrease the loss function. Therefore, any algorithm that can find a second-order stationary point can converge globally for such nonconvex problems. We will review recent algorithmic developments that can efficiently escape (strict) saddle points and find second-order stationary points, including stochastic and perturbed gradient descent, trust-region methods, and so on. These approaches do not require special initializations.

{\em Initialization and local refinement:} The second approach starts with a careful initialization that lands into a reasonable neighborhood of the ground truth (global optima), and then applies local refinements using simple, iterative algorithms such as gradient descent and alternating minimization. The loss function, in a proximity of the global optima, may behave like a (strongly) convex function, which enables fast convergence of the algorithm. 


